Unsynthesizable Cores - Minimal Explanations for Unsynthesizable High-Level Robot Behaviors

With the increasing ubiquity of multi-capable, general-purpose robots arises the need for enabling non-expert users to command these robots to perform complex high-level tasks. To this end, high-level robot control has seen the application of formal methods to automatically synthesize correct-by-construction controllers from user-defined specifications; synthesis fails if and only if there exists no controller that achieves the specified behavior. Recent work has also addressed the challenge of providing easy-to-understand feedback to users when a specification fails to yield a corresponding controller. Existing techniques provide feedback on portions of the specification that cause the failure, but do so at a coarse granularity. This work presents techniques for refining this feedback, extracting minimal explanations of unsynthesizability.

==> cores_overview.tex <==
As mentioned in Section \ref{problem}, when a specification does not yield an implementing automaton, existing algorithms provide feedback of a course granularity \cite{TRO12}. This section describes techniques implemented in this work that provide fine-grained feedback in certain cases by tracing the problem back to a minimal explanation, and identifies the challenges that must be overcome to extend these techniques to the remaining cases.

When controller synthesis fails the specification is called \emph{unsynthesizable}. Unsynthesizable specifications are either \emph{unsatisfiable}, in which case the robot cannot succeed no matter what happens in the environment (e.g., if the task requires patrolling a disconnected workspace), or \emph{unrealizable}, in which case there exists at least one environment that can prevent the desired behavior (e.g., if in the above task, the environment can disconnect an otherwise connected workspace, such as by closing a door). More examples illustrating the two cases can be found in \cite{TRO12}. 

In either case, the robot can fail in one of two ways: either it ends up in a state from which it has no valid moves (termed \emph{deadlock}), or the robot is able to change its state infinitely, but one of its goals is unreachable without violating the specified safety requirements (termed \emph{livelock}). In the context of unsatisfiability, an example of deadlock is when the system safety conditions contain a contradiction within themselves. Similarly, unrealizable deadlock occurs when the environment has at least one strategy for forcing the system into a deadlocked state.  Livelock occurs when there is one or more goals that cannot be reached while still following the given safety conditions. Note that Specification~\ref{spec:unreal1} is a case of livelock: the robot can follow its safety indefinitely by moving between the first four rooms on the left, but is prevented from ever reaching the goal if it sees a person all the time -- the environment is able to disconnect the topology using the person sensor. 

Previous work produced explanations of unsynthesizability in terms of combinations of the specification components (i.e., initial conditions, safeties and goals). However, in many cases, the true conflict lies in small subsections of these formulas.

\begin{spec}
\small
\begin{enumerate}
\item \textit{Don't go to the kitchen} (part of $\varphi_s^t$) \label{item:b0}
\item \textit{Visit the kitchen} (part of $\varphi_s^g$) \label{item:b1}
\item \textit{Always activate your camera} (part of $\varphi_s^t$) \label{item:b2}
\end{enumerate}
\caption{Unsatisfiable specification -- livelock}
\label{spec:unsat1}
\end{spec}

Consider Specification~\ref{spec:unsat1}. It is clear that the safety requirement in (\ref{item:b0}) conflicts with the goal in (\ref{item:b1}), since in order to visit the kitchen one must in fact go there. However, the safety requirement in (\ref{item:b2}) is irrelevant, and should be excluded from any explanation of why this specification is unsatisfiable. However, the algorithm presented in \cite{TRO12} will return the entirely of $\varphi_s^t$ along with the goal of visiting the kitchen, declaring that this goal is in conflict with some subset of the safeties (but not identifying the exact subset). Note that this example is also a case of livelock: the robot can follow its safety indefinitely by staying out of the kitchen, but is prevented from ever reaching its goal of visiting the kitchen. 






==> feedback.tex <==
Once the guilty portions of the LTL formula generated from a task
specification have been identified, the cause of failure must be
presented to the user. This
section describes the two modes of communicating the cause of
unsynthesizability that are deployed in the presented system.

\subsection{Explaining Unsatisfiable Tasks}

Giving users detailed feedback regarding \emph{why} a task is
unachievable is essential to helping them correct it. While better
than simply reporting failure, returning the user a set of LTL
formulas responsible for unsatisfiability is not
enough to help them correct the natural language specification that
generated it. To provide actionable feedback to the user, SLURP uses a
combination of the user's own natural language along with
structured language created during the LTL formula generation process
to explain problems with the specified task.

Consider the example given above where the combination of the
statements ``Don't go to the kitchen'' and ``Visit the kitchen''
results in an unsatisfiable specification. The minimal unsatisfiable
core of the specification consists of the following statements:
\[
\small
\begin{array}{r@{\extracolsep{0.1em}}l}
\G  & (\neg s.kitchen) \\
\G & (\X  s.mem\_visit\_kitchen \Leftrightarrow \\ 
& (s.mem\_visit\_kitchen \vee \X s.kitchen)) \\
\G \F & (s.mem\_visit\_kitchen)
\end{array}
\]

\noindent
To explain the conflict, the system lists the goal that cannot be
satisfied and natural language corresponding to the formulas in the
minimal core. For the specification above, the response is:

\begin{quote}
{\small
The problematic goal comes from the statement `Go to the
kitchen.'. The system cannot achieve the sub-goal ``Visit `kitchen'.''.

The statements that cause the problem are:
\begin{itemize}
\item ``Don't go to the kitchen.'' because of item(s): ``Do not go to `kitchen'.''.
\item `Go to the kitchen.' because of item(s): ``Visit `kitchen'.''.
\end{itemize}
}
\end{quote}

\noindent
Additional examples of feedback are given in Section~\ref{example}.

\subsection{Interactive Exploration of Unrealizable Tasks}
\label{mopsy}
Succinctly summarizing the cause of an unrealizable specification is challenging, sometimes even for a human, 
so our system uses an interactive game (shown in Fig.~\ref{fig:follow_feedback}) to demonstrate an environment behavior that will cause the robot to fail. 
This lets the user attempt to play as a robot against an adversarial environment, and in the process gain insight into the nature of the problem. 
An example of this tool in use is given in Section~\ref{example_unreal}.

At each discrete timestep, the user is presented with the current goal to pursue and the current state of the environment. 
The user is then able to change the location of the robot and the states of its actuators in response.

Earlier versions of this tool simply prevented the user from making any moves that were disallowed by the specification. 
However, by using the core-finding feedback subsystem presented in this work,
a specific explanation is now given about what part of the original specification is in conflict with any invalid moves.
This is done by finding the unsatisfiable core of a single-step satisfiability problem involving the user's current state, the desired next state, and all of the robot's specified safety conditions.



==> relatedRobotics.tex <==
Several recent works have addressed the problem of analyzing high-level specifications that are unsynthesizable. Feedback about the cause of unsynthesizability can be provided to the user in the form of a modified specification \citep{Fainekos11,KimFainekos12}, a highlighted fragment of the original specification \citep{CAV11}, or by allowing the user to interact with an adversarial environment that prevents the robot from achieving the specified behavior \citep{ICRA12,TRO12}. Building upon these approaches, the work presented in this paper provides minimal explanations of unsatisfiable specifications, as described in Section \ref{cores}, and provides fine-grained natural language feedback that is not necessarily just a subset of the original natural language specification. It also enhances the interactive visualization tool with feedback on why particular robot actions may be disallowed in a given state, as described in Section \ref{mopsy}. This work subsumes that presented in \cite{RSS13,IROS13}, and includes additional techniques for identifying unrealizable cores in certain cases, as described in Section \ref{cores_iterate}.



